Linv invariant and $G_2$ web space

In this paper, we reconstruct Kuperberg's $G_2$ web space. We introduce a new web (a trivalent diagram) and new relations between Kuperberg's web diagrams and the new diagram. Using the $G_2$ webs, we define crossing formulas corresponding to R-matrices associated to some $G_2$ irreducible representations and calculate $G_2$ quantum link invariant for some torus links.

==> figure/web-12-12.tex <==
{\unitlength 0.1in%
\begin{picture}(16.0000,16.0000)(2.0000,-20.0000)%
\special{pn 40}%
\special{ar 2400 1000 1000 1000 2.2142974 4.0688879}%
\special{pn 40}%
\special{ar -400 1000 1000 1000 5.3558901 0.9272952}%
\special{pn 40}%
\special{ar 2400 1000 900 900 2.2142974 4.0688879}%
%\special{pn 40}%
%\special{ar -400 1000 900 900 5.3558901 0.9272952}%
\end{picture}}%

